Evaluating the Energy Consumption of Machine Learning: Systematic Literature Review and Experiments

Monitoring, understanding, and optimizing the energy consumption of Machine Learning (ML) are various reasons why it is necessary to evaluate the energy usage of ML. However, there exists no universal tool that can answer this question for all use cases, and there may even be disagreement on how to evaluate energy consumption for a specific use case. Tools and methods are based on different approaches, each with their own advantages and drawbacks, and they need to be mapped out and explained in order to select the most suitable one for a given situation. We address this challenge through two approaches. First, we conduct a systematic literature review of all tools and methods that permit to evaluate the energy consumption of ML (both at training and at inference), irrespective of whether they were originally designed for machine learning or general software. Second, we develop and use an experimental protocol to compare a selection of these tools and methods. The comparison is both qualitative and quantitative on a range of ML tasks of different nature (vision, language) and computational complexity. The systematic literature review serves as a comprehensive guide for understanding the array of tools and methods used in evaluating energy consumption of ML, for various use cases going from basic energy monitoring to consumption optimization. Two open-source repositories are provided for further exploration. The first one contains tools that can be used to replicate this work or extend the current review. The second repository houses the experimental protocol, allowing users to augment the protocol with new ML computing tasks and additional energy evaluation tools.

==> tables/YN-data-based-estimation-model-2018above.tex <==
\paragraph{YN studies in the group ``data-based estimation model''} 
 \label{tab:YN-data-based-estimation-model} 
\begin{longtable}{|>{\raggedright\arraybackslash}p{2.75cm}|p{11.75cm}|p{0.7cm}|}
\toprule
\bfseries study & \bfseries detail & \bfseries cites \\
\midrule 
\endhead
\cite{alavani2023}, 2023, NU & ML model (XGBoost) with code features and minimal runtime information as inputs, for CUDA program on GPU & 1 \\
\cite{pathania2023}, 2023, ESAVE &  (Estimating Server And Virtual machine Energy) ML model (XGBoost) with hardware specifications and CPU utlization as inputs, for bare-metal servers & 0 \\
\cite{wu2022}, 2022, MuMMI &  (Multiple Metrics Modeling Infrastructure) tree/rule-based, nonlinear and linear ML models with PMC as inputs, for CPU and RAM; \textbf{available:} data are available on request from the authors & 2 \\
\cite{shim2022}, 2022, DeepPM &  (Deep Power Meter) ML model (Transformer) with compiled binary as inputs, for CPU & 1 \\
\cite{morlans2022}, 2022, NU & ML model (fully connected NN) with hardware specifications as inputs, for laptops & 0 \\
\cite{shahid2021b}, 2021, NU & linear models with PMC as inputs, for CPU and RAM or GPU & 8 \\
\cite{shahid2021a}, 2021, NU & linear models with PMC as inputs, for CPU and RAM or GPU & 12 \\
\cite{aboubakar2021}, 2021, NU & Statistical model ARIMA (Autoregressive Integrated Moving Average) based on hardware specifications and utilization, for CPU and RAM & 1 \\
\cite{lin2020}, 2020, NU & ML model (based on Elman NN and Long Short Term Memory NN) with PMC as inputs, for server & 40 \\
\cite{kloh2020}, 2020, NU & ML models (Linear Regression, Decision Tree, Support Vector Machine, NN) with PMC as inputs, for CPU, memory, cache, Jetson TX2; \textbf{available:} trained models (no documentation) \href{https://github.com/ViniciusPrataKloh/dissertacao-mestrado}{\ref*{link-kloh2020}} & 4 \\
\cite{karantoumanis2020}, 2020, NU & ML models (Ordinary least squares linear regression, Lasso, Ridge, Epsilon-support vector, Decision tree, Random forest, k-nearest neighbors, Multi-layer Perceptron) with CPU utilization and RAM, Disk and Network information as input, for a scientific application running in a data center; \textbf{available:} some models (in the article) & 1 \\
\cite{fu2018}, 2018, NU & ML model (Ridge regression) with information from the Perf tool as inputs, for CPU, RAM and Disk & 7 \\
\cite{dutta2018}, 2018, NU & ML models (ZeroR, Linear Regression, Sequential Minimal Optimization Regression, K-Nearest Neighbor, Reduced Error Pruning Tree, Bagging, Random Forest, NN) with GPU frequency, memory frequency and hardware resource utilization levels as inputs, for the GPU & 0 \\
\bottomrule
\end{longtable}


==> tables/YN-data-based-estimation-model-2018below.tex <==
\paragraph{YN studies in the group ``data-based estimation model''} 
 \label{tab:YN-data-based-estimation-model} 
\begin{longtable}{|>{\raggedright\arraybackslash}p{2.75cm}|p{11.75cm}|p{0.7cm}|}
\toprule
\bfseries study & \bfseries detail & \bfseries cites \\
\midrule 
\endhead
\cite{jiang2017}, 2017, NU & ML model (Elman Neural Network) with information about the temperature, humidity and hardware utilization as inputs, for a server & 0 \\
\cite{li2016b}, 2016, NU & nonlinear relation between characteristics of a network representing the software and the power used, for CPU, RAM, Network and Disk & 1 \\
\cite{veni2016}, 2016, NU & ML model (Support Vector Regression) with PMC as inputs, for CPU, RAM, Cache and Disk of a virtual machine & 10 \\
\cite{gutierrez2015a}, 2015, NU & ML model (NN) with PMC as inputs, for the CPU & 1 \\
\cite{foo2015}, 2015, NU & ML model (Evolutionary NN) with inputs such as the number of Map and Reduce, CPU utilization and file size, for jobs in cloud data center & 29 \\
\cite{harton2015}, 2015, NU & ML model (Random Forest) with CPU utilization as input, for a whole server & 4 \\
\cite{gutierrez2015b}, 2015, NU & ML model (Feed-forward NN) with PMC as inputs, for CPU & 1 \\
\cite{colmant2014}, 2014, BitWatts & BitWatts - model with PMC as inputs, for processes, accounts for CPU; \textbf{available:} package, code \href{https://github.com/Spirals-Team/bitwatts}{\ref*{link-colmant2014}} & 0 \\
\cite{storlie2014}, 2014, NU & hierarchical Bayesian modeling with hidden Markov and Dirichlet process models, for an HPC job & 18 \\
\cite{kim2014}, 2014, NU & model with operating frequency, number of active cores, number of cache accesses, and number of the last level cache misses as inputs, for CPU and RAM of a server & 26 \\
\cite{singh2013}, 2013, NU & model (Support Vector Machine) with hardware utilization as inputs, for processes on CPU, RAM, I/O and Network & 18 \\
\cite{chen2012}, 2012, ECAT &  (Energy-Consumption-Analysis-Tool) model based on task performance parameters such as CPU utilization, and hardware and software resources allocated, for data-, computation- or communication-intensive task in the cloud & 76 \\
\cite{schubert2012}, 2012, eprof & model with PMC as inputs, and stack trace used for attribution of used energy to code locations, on CPU, RAM, Disk and Network & 71 \\
\cite{zamani2010}, 2010, NU & Autoregressive moving average (ARMA) model with past and present PMC as intputs, for a server with CPUs & 13 \\
\cite{ma2009}, 2009, NU & Support Vector regression model with workload signals as inputs, for GPU & 152 \\
\bottomrule
\end{longtable}


==> tables/YN-data-based-estimation-modelon-chip-sensors.tex <==
\begin{table}[ht!] 
\centering 
\begin{tabular}{|>{\raggedright\arraybackslash}p{2.75cm}|p{11.75cm}|p{0.7cm}|}
\toprule
\bfseries study & \bfseries detail & \bfseries cites \\
\midrule
\bottomrule
\end{tabular}
\caption{YN studies in the group ``data-based estimation modelon-chip sensors''} 
\label{tab:YN-data-based-estimation-modelon-chip-sensors} 
\end{table}
